Adaptive extra-gradient methods for min-max optimization and games

We present a new family of min-max optimization algorithms that automatically exploit the geometry of the gradient data observed at earlier iterations to perform more informative extra-gradient steps in later ones. Thanks to this adaptation mechanism, the proposed method automatically detects whether the problem is smooth or not, without requiring any prior tuning by the optimizer. As a result, the algorithm simultaneously achieves order-optimal convergence rates, i.e., it converges to an $\varepsilon$-optimal solution within $\mathcal{O}(1/\varepsilon)$ iterations in smooth problems, and within $\mathcal{O}(1/\varepsilon^2)$ iterations in non-smooth ones. Importantly, these guarantees do not require any of the standard boundedness or Lipschitz continuity conditions that are typically assumed in the literature; in particular, they apply even to problems with singularities (such as resource allocation problems and the like). This adaptation is achieved through the use of a geometric apparatus based on Finsler metrics and a suitably chosen mirror-prox template that allows us to derive sharp convergence rates for the methods at hand.

==> Algorithms/UniProx.tex <==
%----------------------------------------------------------------------
%%% UNIPROX
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\begin{algorithmic}[1]
\Require
%	number of iterations $\nRuns$,
	Bregman regularizer $\hreg$
\State
	choose $\state_{\halfstart} \neq \state_{\start} \in \points$;
	%set $\res_{\prestart} = \bracks{\breg(\state_{\halfstart},\state_{\start}) + \breg(\state_{\start},\state_{\halfstart})}^{1/2}$
%	$\cumres_{0} = 0$
	\Comment{initialization}%
%\If
%	{$\oper(\state_{\halfstart}) = 0$}
%	\State
%		\Return $\bar\state_{\nRuns} \leftarrow \state_{\halfstart}$
%\Else
\For{$\run = \running, \nRuns-1$}
	\State
		set $\step_{\run} = \parens[\big]{1+\sum_{\runalt=\prestart}^{\run-1} \norm{\oper(\state_{\runalt+1/2})-\oper(\state_{\runalt})}^{2}_{\state_{\runalt+1/2}}}^{-1/2}$
		\Comment{step-size}%
	\State
		get $\signal_{\run} = \oper(\state_{\run})$;\quad
		set $\state_{\run+1/2} = \prox_{\state_{\run}}(-\step_{\run}\signal_{\run})$
		\Comment{leading state}%
	\State
		get $\signal_{\run+1/2} = \oper(\state_{\run+1/2})$;\quad
		set $\state_{\run+1} = \prox_{\state_{\run}}(-\step_{\run}\signal_{\run+1/2})$
		\Comment{update state}%
	%\State
		%set $\res_{\run}^{2} = \bracks{\breg(\state_{\run+1},\state_{\run+1/2}) + \breg(\state_{\run+1/2},\state_{\run+1})}/\step_{\run}^{2} + 1/\run$
		%	\State
%		receive signal $\signal_{\run} \leftarrow -\bracks{\nabla\loss_{\run}(\state_{\run}) + \noise_{\run}}$
%		\Comment{oracle feedback}%
%	\State
%		update $\state_{\run+1} \leftarrow \Eucl(\state_{\run} + \step_{\run}\signal_{\run})$
%		\Comment{gradient step}%
\EndFor
	\State
		\Return $\bar\state_{\nRuns} \leftarrow (1/\sum_{\run=1}^{\nRuns}\step_{\run}) \sum_{\run=\start}^{\nRuns} \step_{\run}\state_{\run+1/2}$
		\Comment{candidate solution}%
%\EndIf
\end{algorithmic}

==> Impact.tex <==
%----------------------------------------------------------------------
%%% IMPACT
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


Our paper is primarily theoretical and, as such, we do not feel that it presents any ethical concerns to the community.
Our main objective was to design an adaptive algorithm for min-max optimization problems and games that simultaneously achieves the following:
\begin{enumerate*}
[\itshape a\upshape)]
\item
%an $\bigoh\parens[\big]{1/\sqrt{\nRuns}}$ convergence rate in non-smooth problems and $\bigoh(1/\nRuns)$ in smooth ones;
order-optimal rates in smooth\,/\,non-smooth problems;
and
\item
convergence beyond the standard boundedness\,/\,Lipschitz continuity conditions.
\end{enumerate*}
The proposed method provides a flexible, freely available toolkit that can prove beneficial to researchers and practitioners in the field, and we do not foresee any ethical concerns arising from its use.
